Learning Reliable Logical Rules with SATNet

Bridging logical reasoning and deep learning is crucial for advanced AI systems. In this work, we present a new framework that addresses this goal by generating interpretable and verifiable logical rules through differentiable learning, without relying on pre-specified logical structures. Our approach builds upon SATNet, a differentiable MaxSAT solver that learns the underlying rules from input-output examples. Despite its efficacy, the learned weights in SATNet are not straightforwardly interpretable, failing to produce human-readable rules. To address this, we propose a novel specification method called "maximum equality", which enables the interchangeability between the learned weights of SATNet and a set of propositional logical rules in weighted MaxSAT form. With the decoded weighted MaxSAT formula, we further introduce several effective verification techniques to validate it against the ground truth rules. Experiments on stream transformations and Sudoku problems show that our decoded rules are highly reliable: using exact solvers on them could achieve 100% accuracy, whereas the original SATNet fails to give correct solutions in many cases. Furthermore, we formally verify that our decoded logical rules are functionally equivalent to the ground truth ones.

==> delete/delete.tex <==
A major line of work combines logic programming with neural networks, learning the associated weight of each logical rule. However, these efforts require define a rule template manually, which is highly non-trivial and time-consuming. 

Bridging logical reasoning and deep learning is a key objective of modern AI systems. In this paper, we introduce a general framework that enables the generation of interpretable and verifiable logical rules through differentiable learning, without the need for pre-specified logical structures. Technically, we adopt the learning framework of SATNet, a differentiable MaxSAT solver that utilizes semidefinite relaxation to learn the underlying logical rules solely from input-output examples. Note that the learned rules in SATNet are not interpretable, we propose a novel specification method, called maximum equality, which translates the internal weight of SATNet into a set of propositional logical rules in MaxSAT form. With the decoded logical rules, we further present a fast verification method that evaluates them against the ground truth rules created by human experts. To evaluate the efficacy of our framework, we conducted experiments on the parity function and 4x4 Sudoku problems. Our results demonstrate that our decoded rules are very robust: using MaxSAT solvers on our generated rules could achieve 100\% accuracy on these tasks, whereas SATNet fails to give the correct solution in some cases. Furthermore, we show that the generated logical rules are functionally equivalent to the ground truth rules, which have a similar solution space. 

Our proposed framework has the potential to significantly enhance the interpretability of SATNet and enable its adoption in real-world applications that require transparent decision-making processes. The ability to learn interpretable logical rules directly from data could pave the way for new advancements in deep learning and logical reasoning integration.

Given the decoded weighted MaxSAT formula, we could call exact solvers for inference, making the solving process transparently. Moreoever, to validate our generated logical rules with the expert-written rules, we further propose a fast verification method that checks the weight of valid solutions of the logical rules around its neighborhood.

We evaluate our proposed framework on the partity function and 4 $\times$ 4 Sudoku problems. Experiments show that our framework achieve 100\% accuracy on these tasks, while SATNet fails at some cases. We further certify this cases and show that this is because SATNet gives suboptimal solution to the learned weighted MaxSAT formula. We also verify the decoded logical rules and prove that our generated rules have similar solution space with the ground-truth ones: the weight of the solutions corresponding the valid solution is the highest around its neighborhood with up to $k$ bits.

The second one is to compare the solution space between our decoded formula and the ground-truth rules written by human experts. Note the entire solution space may be extremely huge, we reduce the space by checking the weight of solution that satisfy the rules around its neighborhood with up to $k$ bits. 

the weight of each valid solution in entire solution space between the decoded weighted MaxSAT formula and the ground-truth rules written by human experts.

empowering the adaptation of ILP to various input types and wider domains.

Inductive logic programming (ILP)~\citep{ilp1,ilp2} is a traditional paradigm for learning explicit logic programs from examples, using a limited set of rule templates. Recently, there have been massive effort to combine neural networks with ILP, empowering the adaptation of ILP to various input types and wider domains.

There are a few limitations to our proposed framework. First, our framework is built upon SATNet, which is only capable of learning propositional logical rules rather than first order or higher order rules. Second, given the variable number $n$, our decoded logical rules may have $\mathcal{O}(n^2)$ clauses in the weighted MaxSAT formula in worst case, which may be time-consuming for an exact solver to solve during inference for very large $n$. We would like to explore other optimization approaches to make the $C$ matrix much sparse and reduce the size of learned rules as future work.


In this work, we present a framework that decodes a set of interpretable logical rules from the learned weight in SATNet. We first show that the optimnization formulation in SATNet is lack of interpretability empirically and theoretically. Then we propose our specification method, maximum equality, that transform the weight of SATNet to a weighted MaxSAT formula. To check the correctness of our decoded formula, we also propose a verfication method that compares the solution space of our generated one and the ground truth. Experiments on the parity function, Sudoku puzzles and string transformation shows that our generated rules are highly robust and verifiable: using exact solvers could achieve full accuracy while SATNet fails to give the right solution for some cases.

first dive into the details of the interpretation in the original formulation of SATNet. Based on the optimization formulation of SATNet, we present our specification approach that decodes a set of logical rules from the weight of SATNet and our verification approach to compare them with the human-written logical rules.

Moreover, we further certify some cases when $S$ fail to represent the ground truth logical rules theoretically. Here, we take the parity function as an example, whose ground truth rules and the corresponding $S$ matrix in SATNet is defied as follows:

The first two variables in the ground truth represent the two input bits and the third variable represents the output bit. However, SATNet additionally defines a truth variable and adds it to each clause in $S$ with negative polarity. This results in $S^TS$ be a zero matrix, leading to collapse of the SDP approach in SATNet. Besides the parity function, other logical rules with the similar symmetric property could cause the same problem. Therefore, the clause matrix $S$ defined in SATNet is lack of interpretability that it is not able to represent a range of logical rules theoretically.



If the clause matrix $S$ can indeed capture the logical rules in the data, it is expected that SATNet can solve all testing problems when $S$ is given as ground truth rules. We investigate whether $S$ has such a representative ability by substituting human-written ground truth rules of $4\times 4$ Sudoku puzzles to $S$ and using SATNet to solve the testing instances.

Despite its potential in capturing the rules, $S$ alone is unable to fully represent the complex logic inherent in the Sudoku puzzles.

\begin{definition}
\label{def:k-bits}
Given any satisfying assignments in the SAT formula, if the weight of its assignment with fixed 


Given any valid input assignments to the ground truth that can determine the assignment of other values uniquely, if each optimal solution of the weighted MaxSAT also correspond to a satisfying assignment in the SAT formula, the two formulas are called unique functional equivalence.
\end{definition}

each satisfying solution in the SAT formula (i.e., a valid instance that satisfies the ground-truth logical rules) has a strictly higher weight than unsatisfying solutions in the weight MaxSAT formula, these two formulas function equivalently. Notably, if the solution space is excessively huge, we reduce the verification space by checking the weight of each valid solution within its neighboring solutions varies in $k$ bits

In short, our contributions are summarized as follows:
\begin{itemize}[noitemsep, topsep=1pt, partopsep=1pt, listparindent=\parindent, leftmargin=*]
\item We propose a novel specification that decodes a set of logical rules in the weighted MaxSAT form from SATNet, enabling interpretable rule learning through differential learning, without using rule templates.
\item We propose several verification approaches to validate the correctness of our decoded rules with human-written rules.
\item Experiments
\item An effective and efficient neuro-symbolic learning framework conducting the neural network training and logical constraint learning simultaneously;
\item Two sensible techniques to support our framework: (1) a trust region method to prevent the degeneracy of logic programming; (2) difference of convex programming for relaxing the logical constraints.
\item Theoretical analysis for the convergence of our framework, as well as empirical evaluation on four tasks demonstrate the superior performance of our framework.
\end{itemize}


. For each input $\s{x_i}$, we fix the assignment of some variables $v_i \in V_\mathcal{I}$ according to the input $x_i$. For each output instance $y_i$, we use them to construct the corresponding variable assignment $v_o \in V_o$.
For each input instances

Given a dataset contains input-output examples of problem $\mathcal{D}(x, y)$

are interested in logical problems that can be reduced as instances of MaxSAT, an analogue of SAT which encompasses a rich domain of symbolic AI. Specifically, given one logical problem, we enumerate the variables $Z=(z_1, z_2,...,z_n)^T\in \{0,1\}^n$ and partition $Z$ into input set $Z_\mathcal{I}$ and $Z_\mathcal{O}$ according to the  specific instance of the problem.

Then we utilize the SATNet~\ref{} to reduce the problem into MaxSAT form. Concretely, we utilize SATNet to construct the Conjunctive Normal Form (CNF) matrix $S\in \mathbb{R}^{m\times n}$, where $m$ denotes the number of clauses in the captured CNF formula and $n$ denotes the number of variables. The output variables $Z_\mathcal{O}$ are computed to maximize the satisfied rows in the $S$ matrix, where the MaxSAT is first reduced to the SDP optimization problem and mixing method~\ref{} is adopted to solve this SDP relaxation. 

One application of this formulation is Sudoku, a problem draws much attention of researchers recently. We consider Sudoku of board size $4$, where $Z$ represents the assignment of each cell. $Z_\mathcal{I}$ and $Z_\mathcal{O}$ are partitioned according to the assignment of which cell is given and which is masked, and $\mathcal{I}+\mathcal{O}=64$. Specifically, $z_{i,j.k}=1$ denotes we assign the $i$-th row and the $j$-th column cell value $k$, and $z_{i,j.k}=0$ otherwise.

SATNet can be levergerd to model a rich class of logical problems. Nevertheless, each element of the $S$ matrix is a real number, which contradicts the assumption from SATNet's original formulation that the $S$ matrix contains only $1,-1$ and $0$, which limits the explicit interpretation of the $S$ matrix of logical rules and impede widespread applications of real-world problems. 

In this work, we novely introduce a framework which addressess the of interpretability limitation of SATNet and leverages a novel formulation called maximum equality to transform the learned matrix $C=S^TS$ into a weighted MaxSAT formula. 

For the inference in SATNet, each relaxed variable vector $v_i$ will be assigned to a probabilistic value according to its angle between the truth vector $v_{\top}$ and then rounded to a Boolean value $z_i$ with a threshold value of 0.5. We can summarize such a procedure to the following optimization problem:

\begin{equation}
    \operatorname*{arg\,min}_{V\in\mathbb{R}^{k\times n}}\langle C, V^TV\rangle \quad\text{s.t.}\ \left\|v_i \right\|=1 \text{ for } i\in [1,n].
\end{equation}
This is equivalent to optimizing the following equation:


It is also worthnoting that any pro

Note that any propositional formula can reduce to Max2SAT using some auxiliary variables, to let our maximum equality represent any formula, we also need to introduce enough auxiliary variables.

To address this issue and reduce the size of the generated rules, we propose a modification to the SATNet implementation. In our modified approach, we directly learn the matrix $C$ in SATNet and apply an iterative hard thresholding algorithm~\citep{iht1,iht2} at each iteration to sparsify the matrix $C$ without compromising the learning performance. This iterative process helps in reducing the density of $C$ and, consequently, the number of clauses in the resulting weighted MaxSAT formula.

To reduce the size of our generated rules, we modify the implementation of SATNet that directly learns the $C$ matrix and further uses an iterative hard thresholding algorithm~\citep{iht1,iht2} to make $C$ becomes sparser at each iteration, without harming the learning performances. Specifically, at each epoch, we uses a theshould function

given input and output variables $Z=[Z_\mathcal{I},Z_\mathcal{O}]$, $|\mathcal{I}|+|\mathcal{O}|=n$, the problem is modeled as a MaxSAT problem and represened with the $S$ matrix, where $S$ is interpreted as a CNF. 


% \subsection{rewrite}
% To begin understanding SATNet~\ref{}, it is recommended to study its precursor, the mixing method~\ref{}. The mixing method is an effective algorithm for resolving semidefinite programming problems that include diagonal constraints. Consider a symmetric matrix $C \in \mathbb{R}^{n \times n}$, where $n,k\in \mathbb{N}$. The optimization problem that the mixing method aims to solve is as Eq.~\ref{eq:sdp}:
% \begin{equation}
%     \operatorname*{arg\,min}_{V\in\mathbb{R}^{k\times n}}\langle C, V^TV\rangle \quad\text{s.t.} \left\|v_i \right\|=1 \text{ for } i\in [1,n]
%     \label{eq:sdp}
% \end{equation}
% where $v_i$ denotes the $i$-th column of matrix $V$, $\langle \cdot \rangle$ denotes the trace operator and  $\left\|\cdot\right\|$ denotes the $L_2$ norm. The mixing method adopts the coordinate descent algorithm to solve this SDP problem. Specifically, each column $v_i$ of $V$ is updated as Eq.~\ref{eq:forward}:
% \begin{equation}
%     v_i = \operatorname*{normalize}(-\sum_{j=1}^n c_{ij}v_j)
%     \label{eq:forward}
% \end{equation}
% The mixing method has been shown to find the optimal solution for the SDP given $k > \sqrt{2n}$~\ref{}.

% MaxSAT is a combinatorial optimization problem that aims to find a satisfying assignment for a Boolean formula with the maximum number of satisfied clauses. Specifically, let $z_1,z_2,...,z_n$ be $n$ Boolean variables, $S_1,S_2,...,S_m$ be $m$ disjunctive clauses of some variables with or without negation: $S_i = \vee_{j=1}^{l^-}\neg z_{i_j} \vee_{j=l^-+1}^{l} z_{i_j}$, where $l^-$ denotes the number of negation literals, and $l$ denotes the total literals. MaxSAT aims to find the assignment that maximizes the number of satisfied clauses.

% To adopt the mixing method to solve the MaxSAT problem, we consider the relaxation form of the MaxSAT~\ref{}. We encoder the Boolean variables as $v_1, v_2,...,v_n$, where $v_i \in \mathbb{R}^k$ and $ \left \|v_i \right\| =1\text{ for }i=1,2,...,n$. We also introduce one logical rule matrix $S\in \mathbb{R}^{m\times n}$, which represents the disjunctive clauses. Specifically, the $i$-th role encodes $S_i$. $S_{ij}=1$ if $S_i$ contains $z_j$; $S_{ij}=-1$ if $S_i$ contains $\neg z_j$; $S_{ij}=0$ otherwise. Then the MaxSAT problem is reduced to the SDP optimization problem defined in Eq.~\ref{eq:sdp}, with $C=S^TS$.

% % The question now is that since we understand how to find solutions for MaxSAT effectively, how can we reduce the specific problem into MaxSAT form and find the conjunction norm form i.e. $S$ matrix? Here
% Furthermore, we introduce SATNet~\ref{}, a differentiable MaxSAT solver that can learn the logical rules of problems that can be reduced to the MaxSAT problem. Concretely, the columns of $V\in \mathbb{R}^{k\times n}$ can be split into two disjoint sets, $\mathcal{I}$ and $\mathcal{O}$. The input Boolean variables $z_i$ are reduced to $v_i$ and $i\in \mathcal{I}$, while the output Boolean variables $z_o$ are rounded from $v_o$ and $o\in \mathcal{O}$.

% Initially, the logical rule matrix $S$ is randomly initialized. Given the input Boolean variables, SATNet encodes each $z_i$ as $v_i$ and adopts Eq.~\ref{eq:forward} to compute $v_o$. SATNet additionally introduces one randomly initialized truth vector $v_{\top}$ s.t. $\left\|v_{\top}\right\|=1$, to represent the truth direction. $z_o$ is rounded as $\cos^{-1}(-v_o^Tv_{\top})/\pi$.

% One import feature of SATNet is differentiable, which enables SATNet to be integrated into deep learning systems. That is, given loss function $l$ and derivatives $\partial l/\partial z_o$, $o \in \mathcal{O}$, SATNet provides an algorithm to compute $\partial l /\partial S$ and $\partial l / z_\mathcal{I}$.

% Let $C=S^TS\in \mathbb{R}^{n\times n}$, $U\in \mathbb{R}^{k\times n}$ with input columns $U_{\mathcal{I}}=0$, $P_o=I_k-v_ov_o^T\in \mathbb{R}^{k\times k}$, $o\in \mathcal{O}$ and $P=\operatorname{vec}(P_o)$.

% For each $o \in \mathcal{O}$, $\partial l / \partial v_o$ is calculated as Eq.~\ref{eq:dvo} 
% \begin{equation}
%     \label{eq:dvo}
%     \frac{\partial l}{\partial v_o}
%     =\frac{\partial l}{\partial z_o}\frac{\partial z_o}{\partial v_o} =\frac{\partial l}{\partial z_o}\frac{v_{\top}}{\pi\sin(\pi z_o)}
% \end{equation}
% The output columns of U can be written as a linear system as Eq.\ref{eq:U}
% \begin{equation}
%     \label{eq:U}
%     \operatorname{vec}(U_{\mathcal{O}})=\left (P\left (\left (\operatorname{diag}\left (\left\|g_o\right\|\right )+C\right )\otimes I_k\right )P\right )^\dagger \operatorname{vec}\left (\frac{\partial l}{\partial \operatorname{vec}(V_\mathcal{O})}\right )
% \end{equation}

% $\partial l /\partial S$ and $\partial l / z_\mathcal{I}$ can be calculated as Eq.~\ref{eq:ds&dvin}.
% \begin{equation}
% \label{eq:ds&dvin}
%     \begin{aligned}
%         \frac{\partial l}{\partial S} &= -\left (V^TU+U^TV \right )S \\
%         \frac{\partial l}{\partial z_i}&=\left (\frac{\partial v_i}{\partial z_i} \right )^T \left (\sum_{o\in \mathcal{O}}u_os_o^T \right )s_i \text{, for } i \in \mathcal{I} \\
%     \end{aligned} 
% \end{equation}
% where $\frac{\partial v_i}{\partial z_i}=\pi \left (\sin (\pi z_i)v_{\top}+\cos (\pi z_i)(I_k-v_\top v_\top^T)v_i^{rand} \right )$.


SATNet computed $Z_\mathcal{O}$ based on the $S$ matrix and $Z_\mathcal{I}$. Let $z$ denotes each column of $Z$. $z_i$ is first relaxed into a continuous vector $v_i\in \mathbb{R}^{k}$ s.t. $\left \| v_i \right \|=1$ for $i=1,...,n$, which can be formularized as:
\begin{equation}
    v_i=-\cos(\pi z_i)v_\top + \sin(\pi z_i)(I_k-v_\top v_\top^T)v_i^{rand}
\end{equation}
where $v_\top\in \mathbb{R}^k$ is a randomly initialized vector representing the truth direction, with constraint $\|v_\top\|=1$.
The relation between continuous vector $v_i$ and discrete variable $z_i$ is $p(z_i=1)=\cos ^-1\left (-v_i^Tv_\top\right)/\pi$.
% \begin{equation}
%     p(z_i=1)=\cos ^-1\left (-v_i^Tv_\top\right)/\pi
% \end{equation}
With the above relaxation, MaxSAT formula can be rewritten as an SDP optimization formula:
\begin{equation}
\label{eq:sdp}
    \mathop{minimize}\limits_{V\in \mathbb{R}^{k\times n}}\langle S^TS, V^TV \rangle \text{ s.t. }\left \| v_i\right \|=1, i=\top, 1,...,n
\end{equation}
We set $k=\sqrt{2n}+1$, since it has been shown the solution $V$ can recover the optimal solution of its relevant SDP given $k>\sqrt{2n}$.~\ref{}. To find the optimal solution of Eq.~\ref{eq:sdp}, the mixing method~\ref{} is applied, which adopts the coordinate descent algorithm: 
\begin{equation}
v_o=-g_o/\left \|g_o \right\|,\text{ where }g_o=VS^Ts_o-\left\|s_o\right\|^2v_o, \text{ for }o\in \mathcal{O}
\end{equation}
The updates are repeated until convergence. 

One import feature of SATNet is differentiable, which enables back propagation in SATNet and makes end-to-end training possible. That is, given loss function $L$ and derivatives $\partial L/\partial Z_\mathcal{O}$, SATNet provides an algorithm to compute $\partial L /\partial S$ and $\partial L / Z_\mathcal{I}$. This feature enables SATNet to be integrated into deep learning systems.



\clearpage
SATNet computed $Z_\mathcal{O}$ based on the $S$ matrix and $Z_\mathcal{I}$. Let $z$ denotes each column of $Z$. $z_i$ is first relaxed into a continuous vector $v_i\in \mathbb{R}^{k}$ s.t. $\left \| v_i \right \|=1$ for $i=1,...,n$, which can be formularized as:
\begin{equation}
    v_i=-\cos(\pi z_i)v_\top + \sin(\pi z_i)(I_k-v_\top v_\top^T)v_i^{rand}
\end{equation}
where $v_\top\in \mathbb{R}^k$ is a randomly initialized vector representing the truth direction, with constraint $\|v_\top\|=1$.
The relation between continuous vector $v_i$ and discrete variable $z_i$ is $p(z_i=1)=\cos ^-1\left (-v_i^Tv_\top\right)/\pi$.
% \begin{equation}
%     p(z_i=1)=\cos ^-1\left (-v_i^Tv_\top\right)/\pi
% \end{equation}
With the above relaxation, MaxSAT formula can be rewritten as an SDP optimization formula:
\begin{equation}
\label{eq:sdp}
    \mathop{minimize}\limits_{V\in \mathbb{R}^{k\times n}}\langle S^TS, V^TV \rangle \text{ s.t. }\left \| v_i\right \|=1, i=\top, 1,...,n
\end{equation}
We set $k=\sqrt{2n}+1$, since it has been shown the solution $V$ can recover the optimal solution of its relevant SDP given $k>\sqrt{2n}$.~\ref{}. To find the optimal solution of Eq.~\ref{eq:sdp}, the mixing method~\ref{} is applied, which adopts the coordinate descent algorithm: 
\begin{equation}
v_o=-g_o/\left \|g_o \right\|,\text{ where }g_o=VS^Ts_o-\left\|s_o\right\|^2v_o, \text{ for }o\in \mathcal{O}
\end{equation}
The updates are repeated until convergence. 

One import feature of SATNet is differentiable, which enables back propagation in SATNet and makes end-to-end training possible. That is, given loss function $L$ and derivatives $\partial L/\partial Z_\mathcal{O}$, SATNet provides an algorithm to compute $\partial L /\partial S$ and $\partial L / Z_\mathcal{I}$. This feature enables SATNet to be integrated into deep learning systems.



%However, an immediate challenge arises from the fact that the ground truth rules are typically given as first-order logic (FOL) rules with quantifiers, while our decoded rules are in the weighted maximum equality (or equivalently MaxSAT form) and may involve auxiliary variables. Completely addressing this challenge is beyond the scope of this work. In this work, we assume quantifiers can be properly eliminated, and ground truth rules can then be encoded as an SAT formula. 

% This discrepancy makes it difficult to define a straightforward notion of correctness.

This accuracy gap can be attributed to the SDP relaxation employed by SATNet, which introduces some errors during the solving process.

% equivalence between an SAT formula and a MaxSAT formula is not well-defined. 
% there is still a non-trivial gap between an SAT formula and a MaxSAT formula, although the latter is indeed a generalization of the former. The equivalence be

% However, the ground truth rules are always written as a SAT formula, and our decoded rules are in the weighted MaxSAT form involving some auxiliary variables, making the definition of correctness not straightforward. 

% Here, we first introduce several definitions to define the equivalence between a weighted MaxSAT formula and an SAT formula.

With ground truth expressed in an SAT formula, the correctness of a learned MaxSAT formula is still not obvious at all, given that 1) the general equivalence between an SAT formula and a MaxSAT formula is not well-defined; and 2) the learned MaxSAT formula may consist of auxiliary variables, which are not used in the ground truth. 

\footnote{add a footnote to refer experimental evaluation}

%It is noteworthy that the unique functional equivalence checking does not have to explicitly enumerate all possible functionally dependent IO pairs. An interesting future work is to design an efficient decision procedure for checking unique functional equivalence between an SAT formula and a (learned) weighted MaxSAT formula. 

% This definition is defined based on the Definition~\ref{def:afe}. Instead of checking all possible valid inputs, we reduce the input space to those that can directly determine the value of other variables.

and each sample contains two $0$-$1$ strings and associated labels (carry bit and output bit).


Since the valid input space of the $4\times 4$ puzzles is really huge, we check whether our learned rules have the unique functional equivalence. We successfully that our maximum equality formula has the unique functional equivalence with the human-written rules. This shows that our decoded rules are highly robust, although SATNet would introduce some error during approximate solving process.

% \paragraph{Evaluations.} 
% All three tasks take input variables sequentially and the model predicts the output variables, which will be compared with the ground truth labels during training and taken as next auxiliary input variables for the model during testing. Concretely, given input streams $z_1, z_2, ..., z_n$ and auxiliary variables $a=\in \{0,1\}^k$ (which will be initialized to $0_k$), our model will capture the first $l$ input variables $z_1, ..., z_l$ and $a$ as input and predict the output variables $o=[o_1, ..., o_k]\in [0,1]^k$. During training, we compute the difference of the stream outputs and their associated labels, e.g. binary cross-entropy and compute the gradients for back propagation. During testing, we round the outputs $o$ to $\{0,1\}^k$ based on the value of each element and the threshold (we set $0.5$ in this experiment). If all the predictions in one stream are correct, we view it a successful prediction.

We perform experiments on both the parity function and $4\times 4$ Sudoku puzzles. When providing the ground truth rules to $C$, SATNet successfully solves the parity function perfectly and achieves an accuracy of $90.45\%$ on the Sudoku dataset, significantly surpassing the accuracy obtained when using the $S$ matrix directly. The accuracy gap between the full accuracy and the achieved one can be attributed to the SDP relaxation employed by SATNet, which introduces some errors during the solving process. 

%
%Notably, if the valid input space is excessively huge, we reduce the verification space by selectively checking the partial inputs that lead to a unique satisfying assignment in the ground truth rules.

there is a factor $2$ for each weight $c_ij$ when transforming Equation~\ 
equality function between two Boolean values 


% In Equation~\ref{eq:maximum_equality}, we apply the equality function to each pair of variable assignments $(z_i, z_j)$ and maximize the overall values according to each weight $-2c_{ij}$. Equation~\ref{eq:reformulation} relaxes the Boolean variables to unit vectors and converts the equality function to the dot product of two variable vectors. Thus, SATNet can also be viewed as a relaxation of optimizing Equation~\ref{eq:maximum_equality} as well. We refer to Equation~\ref{eq:maximum_equality} as the maximum equality formulation, as it maximizes the weighted equality function of assignment pairs.

% to check the solution space between the SAT formula and the weighted MaxSAT formula. Given any valid input to the ground truth rules, it can give us a valid assignment to other variables that satisfies the rules. Similarly, if any valid input to the weighted MaxSAT formula, the optimal solution is also a valid assignment in the SAT formula (no matter what assignments of the auxiliary variables), these two formula functions equivalently.

% \item We prove that propositional logical rules and numerical weights are essentially interchangeable using our proposed interpretation. When necessary, one form can be flexibly reduced into the other. 



%The rest of the paper is organized as follows: Section~\ref{sec:background} formulates the problem and offers detailed background on SATNet. Section~\ref{sec:method} details the uninterpretability of the original SATNet and introduces our proposed maximum equality formulation for generating interpretable logical rules, followed by our verification method for validating the decoded rules. Section~\ref{sec:experiments} presents our experimental evaluations. Section~\ref{sec:related_work} revisits the related work in the field of logical reasoning and deep learning. Section~\ref{sec:conclusion} discusses the limitations and potential future work before concluding the paper.

\footnote{We try both normalized and unnormalized versions of $S$ and report the best result.}

% \begin{equation*}
% \begin{aligned}
% &h\ (\neg a \lor \neg b \lor d)\ \land \ 
% h\ (a \lor b \lor d)\ \land \ 
% h\ (\neg a \lor b \lor \neg d)\ \land \ 
% h\ (a \lor \neg b \lor \neg d)\ \land \\
% &w\ (d) \ \text{if}\ w > 0,\ \text{else} \ w\ (\neg d),
% \end{aligned}
% \end{equation*}

In this work, we investigate one case of incorporating simple domain knowledge after the training but before the inference, which we call \textit{weight repair}.

% It is also noteworthy that the original experiment in SATNet~\citep{satnet} implicitly imposes additional ``one-hot'' constraints by using softmax to enforce that each group of variables corresponding to the same cell has exactly one value of 1 during inference. However, in our experiments, we discard these constraints and instead round all variable values based on a threshold for both SATNet and SATNet*.
